Neural Generative Question Answering

This paper presents an end-to-end neural network model, named Neural Generative Question Answering (GENQA), that can generate answers to simple factoid questions, based on the facts in a knowledge-base. More specifically, the model is built on the encoder-decoder framework for sequence-to-sequence learning, while equipped with the ability to enquire the knowledge-base, and is trained on a corpus of question-answer pairs, with their associated triples in the knowledge-base. Empirical study shows the proposed model can effectively deal with the variations of questions and answers, and generate right and natural answers by referring to the facts in the knowledge-base. The experiment on question answering demonstrates that the proposed model can outperform an embedding-based QA model as well as a neural dialogue model trained on the same data.

==> macros.tex <==
% Math symbols
\newcommand{\real}{\ensuremath{\mathbb{R}}}
\newcommand{\nat}{\ensuremath{\mathbb{N}}}
\newcommand{\irrat}{\ensuremath{\mathbb{I}}}
\newcommand{\rat}{\ensuremath{\mathbb{Q}}}
\newcommand{\comp}{\ensuremath{\mathbb{C}}}
\newcommand{\integer}{\ensuremath{\mathbb{Z}}}
\newcommand{\pr}{\ensuremath{\mathbb{P}}}
\newcommand{\vleq}{\ensuremath{\preceq}}
\newcommand{\vgeq}{\ensuremath{\succeq}}
\newcommand{\vle}{\ensuremath{\prec}}
\newcommand{\vge}{\ensuremath{\succ}}
\newcommand{\gradient}{\nabla}
\newcommand{\Epsilon}{\LARGE \varepsilon}
\newcommand{\spd}[1]{\mathbf{S}^{#1}_{++}}
\newcommand{\symm}[1]{\mathbf{S}^{#1}}
\newcommand{\diag}[1]{\mathbf{diag}(#1)}
\newcommand{\dist}{ \ensuremath{\sim} }
\newcommand{\set}[1]{\{#1\}}
\newcommand{\floor}[1]{\ensuremath{\lfloor#1\rfloor}}
\newcommand{\ceil}[1]{\ensuremath{\lceil#1\rceil}}
\newcommand{\X}{\textbf{X}}
\newcommand{\deltahat}{\ensuremath{\hat{\delta}}}
\newcommand{\tuple}[1]{\ensuremath{\langle#1\rangle}}
\newcommand{\con}{\wedge}
\newcommand{\dis}{\vee}
\newcommand{\sq}[1]{\ensuremath{\left[#1\right]}}
\newcommand{\defn}{\ensuremath{\triangleq}}
\newcommand{\II}{\mathcal{I}}
\newcommand{\mle}{\ll}

% Text format
\newcommand{\bld}[1]{\textbf{#1}}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}
\newcommand{\algo}[1]{\textsc{#1}}
\newcommand{\scaption}[1]{\caption{\algo{#1}}}

% Abbreviations
\newcommand{\todo}[1]{\red{\footnote{#1}}}
\newcommand{\dsum}[2]{\displaystyle\sum_{#1}^{#2}}
\newcommand{\tr}{\textbf{tr }}
\newcommand{\numreset}{\setcounter{equation}{0}}
\newcommand{\eop}{\ensuremath{\ \square}}
\newcommand{\argmax}{\text{argmax}}
\newcommand{\argmin}{\text{argmin}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\note}{\paragraph*{Note}}
\newcommand{\mode}[1]{\text{mode}(#1)}

